LEMMo-Plan: LLM-Enhanced Learning from Multi-Modal Demonstration for Planning Sequential Contact-Rich Manipulation Tasks

Large Language Models (LLMs) have gained popularity in task planning for long-horizon manipulation tasks. To enhance the validity of LLM-generated plans, visual demonstrations and online videos have been widely employed to guide the planning process. However, for manipulation tasks involving subtle movements but rich contact interactions, visual perception alone may be insufficient for the LLM to fully interpret the demonstration. Additionally, visual data provides limited information on force-related parameters and conditions, which are crucial for effective execution on real robots. In this paper, we introduce an in-context learning framework that incorporates tactile and force-torque information from human demonstrations to enhance LLMs' ability to generate plans for new task scenarios. We propose a bootstrapped reasoning pipeline that sequentially integrates each modality into a comprehensive task plan. This task plan is then used as a reference for planning in new task configurations. Real-world experiments on two different sequential manipulation tasks demonstrate the effectiveness of our framework in improving LLMs' understanding of multi-modal demonstrations and enhancing the overall planning performance.

==> config/symbols.tex <==

\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{sansmath}

% character definition
\mathchardef\mhyphen="2D   % define "math hyphen"

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

% equivalence relations
\newcommand{\defeq}{\vcentcolon=}

% maths
\newcommand{\R}     {\mathbb{R}}          % real numbers
\newcommand{\T}     {\mathsf{T}}                % transpose
\newcommand{\transpose}{\mathsf{T}}
\newcommand{\intd}  {\mathrm{d}}          % variable of integration

\newcommand{\bnabla}{\boldsymbol{\nabla}} % (bold) derivative
\newcommand{\gaussian}     {\mathcal{N}}         % Gaussian distribution
\newcommand{\uniform}     {\mathcal{U}}         % uniform distribution

%\newcommand{\be}    {\mathbf{e}}          % basis vector

% bold
\newcommand{\bO}    {\boldsymbol{0}}      % (bold) zero
\newcommand{\bl}    {\boldsymbol{1}}      % (bold) one
\newcommand{\bA}     {\mathbf{A}}         % constraint matrix
\newcommand{\bB}     {\mathbf{B}}         % constraint matrix
\newcommand{\bC}     {\mathbf{C}}         % constraint matrix
\newcommand{\bD}     {\mathbf{D}}         % constraint matrix
\newcommand{\bF}     {\mathbf{F}}         % constraint matrix
\newcommand{\bG}     {\mathbf{G}}         % constraint matrix
\newcommand{\bH}     {\mathbf{H}}         % constraint matrix
\newcommand{\bI}     {\mathbf{I}}          % identity matrix
\newcommand{\bJ}     {\mathbf{J}}         % constraint matrix
\newcommand{\bK}     {\mathbf{K}}         % constraint matrix
\newcommand{\bL}     {\mathbf{L}}         % constraint matrix
\newcommand{\bM}     {\mathbf{M}}         % constraint matrix
\newcommand{\bN}     {\mathbf{N}}         % constraint matrix

\newcommand{\bP}     {\mathbf{P}}         % constraint matrix
\newcommand{\bQ}     {\mathbf{Q}}         % constraint matrix

\newcommand{\bX}     {\mathbf{X}}         % input data matrix
\newcommand{\bY}     {\mathbf{Y}}         % output data matrix
\newcommand{\bW}     {\mathbf{W}}         % output data matrix

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}     {\mathbf{b}}         % constraint vector
\newcommand{\bc}     {\mathbf{c}}         % constraint vector
\newcommand{\be}{\mathbf{e}}
\newcommand{\f}     {\mathbf{f}} 
\newcommand{\bg}{\mathbf{g}}        % (bold) force
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}     {\mathbf{q}}         % (bold) joint angles
\newcommand{\br}     {\mathbf{r}}         % (bold) end-effector positions
\newcommand{\bu}  {\mathbf{u}}          % (bold) commands
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}     {\mathbf{x}}         % (bold) state
\newcommand{\by}     {\mathbf{y}}         % (bold) output/observation
\newcommand{\bz}     {\mathbf{z}}

\newcommand{\bpsi}{\boldsymbol{\psi}}

\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
% parameters
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\btheta}  {\boldsymbol{\theta}}               % parameter vector
%\newcommand{\ntheta}  {p}                                 % index for parameter vector elements
%\newcommand{\dimtheta}{\mathcal{\MakeUppercase{\ntheta}}} % parameter dimensionality
\newcommand{\bxi}{\boldsymbol{\xi}}

% functions
\newcommand{\estimated} [1]{\hat{#1}}
\newcommand{\normalised}[1]{\tilde{#1}}
\newcommand{\optimal}   [1]{\bar{#1}}
\newcommand{\pinv}      [1]{{#1}^\dagger}
\newcommand{\vectornorm}[1]{||#1||}
% \newcommand{\trace}     [1]{\mathrm{Tr}[#1]}        % pseudoiverse quantity
\newcommand{\leftexp}   [2]{{\vphantom{#2}}^{#1}{#2}}

% indices
\newcommand{\nk}      {k}                              % index for roll outs
\newcommand{\Nk}      {\mathcal{\MakeUppercase{\nk}}}  % no. roll outs

% kinematics

%\newcommand{\bJ}     {\mathbf{J}}         % Jacobian
\newcommand{\qdot}   {\dot{q}}            % joint velocities
\newcommand{\bqdot}  {\dot{\bq}}          % (bold) joint velocities
\newcommand{\brdot}  {\dot{\br}}          % (bold) end-effector velocities
\newcommand{\ebq}    {\estimated{\bq}}    % (bold) estimated joint angles
\newcommand{\ebqdot} {\estimated{\bqdot}} % (bold) estimated joint velocities

% dynamics

\newcommand{\qddot}  {\ddot{q}}           % joint accelerations
\newcommand{\bqddot} {\ddot{\bq}}         % (bold) joint accelerations
\newcommand{\bqdddot} {\dddot{\bq}}
%\newcommand{\btau}   {\boldsymbol{\tau}}  % (bold) joint torques
\newcommand{\ebqddot}{\estimated{\bqddot}}% (bold) estimated joint accelerations
\newcommand{\ebtau}  {\estimated{\btau}}  % (bold) estimated joint torques
\newcommand{\rddot}  {\ddot{r}}           % end-effector accelerations
\newcommand{\brddot} {\ddot{\br}}         % (bold) end-effector accelerations
%\newcommand{\bK}     {\mathbf{K}}         % (bold) stiffness matrix
%\newcommand{\bB}     {\mathbf{B}}         % (bold) damping matrix
\newcommand{\brO}    {\br_{0}}            % (bold) equilibrium position in Cartesian space

\newcommand{\kinetic}{\mathcal{K}}
\newcommand{\potential}{\mathcal{U}}
%\newcommand  {\nq}         {n}                   % index for elements of joint position/angle vector
\newcommand  {\dimq}  {\mathrm{n}} % joint position/angle dimensionality
\newcommand{\ntheta}     {m}                   % index for elements of motor position/angle vector
\newcommand{\dimtheta}{\mathrm{{d_m}}}
\newcommand{\dimx}{\mathrm{d_x}}
\newcommand{\dimu}{\mathrm{m}}
%\newcommand  {\dimu}{\mathcal{\MakeUppercase{\nu}}} % action dimensionality

%\newcommand  {\f}          {\bm{f}}              % (bold) state space dynamics
\renewcommand{\btheta}     {\boldsymbol{\theta}} % (bold) motor position/angle
\newcommand  {\bthetadot}  {\dot{\btheta}}       % (bold) motor velocity
\newcommand  {\bthetaddot} {\ddot{\btheta}}      % (bold) motor accelerations
\newcommand  {\bthetadddot}{\dddot{\btheta}}     % (bold) motor jerk
\newcommand  {\thetad}     {\theta_d}            % (bold) desired motor position/angle
\newcommand{\thetadot}{\dot{\theta}}
\newcommand{\thetaddot}{\ddot{\theta}}
\newcommand{\thetadddot}{\dddot{\theta}}


% optimal control
\newcommand  {\dt}         {\,\intd t}             % t as variable of integration
%\renewcommand{\nu}  {q}                   % index for elements of u
\newcommand  {\bpi} {\boldsymbol{\pi}}    % (bold) control policy
\newcommand  {\bxdot}{\dot{\bx}}          % (bold) state velocities

\newcommand{\U}          {U}                   % set of admissible controls

% reinforcement learning






% cost function
\newcommand  {\C}{J}         % {\MakeUppercase{\c}}  % cost
\newcommand{\cost}          {l}                   % instantaneous cost
\newcommand  {\costt}         {\cost_t}                % instantaneous task cost
\newcommand  {\coste}         {\cost_e}                % instantaneous energy cost

\newcommand  {\cT}{H}         % {\MakeUppercase{\c}}  % terminal cost

\newcommand  {\Ct}         {\C_t}                % integral of accuracy cost
\newcommand  {\Ce}         {\C_e}                % integral of energy cost
\newcommand  {\we}          {w_e}                   % cost trade-off parameter for energy term
\newcommand  {\eps}        {\epsilon}            % cost regularisation parameter

% 
\newcommand  {\W}          {W}                   % mechanical work
\newcommand  {\Wn}         {\overline{\W}}       % net mechanical work
\newcommand{\inertia}{m} % inertia
\newcommand{\stiffness}{K}
\newcommand{\damping}{D}
\newcommand{\energy}{E}
\newcommand{\Es}{E_s}


\newcommand{\powerin}{P_{\mathrm{in}}}
\newcommand{\powerout}{P_{\mathrm{out}}}
\newcommand{\powerinone}{P_{\mathrm{in1}}}
\newcommand{\powerintwo}{P_{\mathrm{in2}}}
\newcommand{\Prege}{P_\mathrm{rege}}
\newcommand{\Erege}{E_\mathrm{rege}}
\newcommand{\Ein}{E_\mathrm{in}}
\newcommand{\Enet}{E_\mathrm{net}}




\newcommand{\ls}{l_s}
\newcommand{\finaltime}{t_f}

\newcommand{\DCr}{D_r}
\newcommand{\DCd}{D_d}

\newcommand{\motorone}{\mathrm{M}_1}
\newcommand{\motortwo}{\mathrm{M}_2}

\newcommand{\taumotorone}{\tau_{m1}}
\newcommand{\taumotortwo}{\tau_{m2}}
\newcommand{\thetamotorone}{\theta_1}
\newcommand{\thetamotortwo}{\theta_2}

\newcommand{\Pd}{P_d}

\newcommand{\transRege}{\alpha}

% inputs/outputs

%\newcommand{\nx}     {p}                  % index for elements of input/state vector
%\newcommand{\dimx}   {\mathcal{\MakeUppercase{\nx}}} % input/state dimensionality

%\newcommand{\ny}     {r}                  % index for elements of output/observation vector
%\newcommand{\dimy}   {\mathcal{\MakeUppercase{\ny}}} % output/observation dimensionality

% learnt models
%\newcommand{\bm}     {\mathbf{m}}         % (bold) RBF or local model centres
%\newcommand{\bxn}    {\bx_{\nd}}          % nth input data point
%\newcommand{\byn}    {\by_{\nd}}          % nth output data point





% constrained systems

%\newcommand{\nb}     {s}                  % index for elements of b
%\newcommand{\dimb}   {\mathcal{\MakeUppercase{\nb}}} % observation dimensionality
%\newcommand{\bN}     {\mathbf{N}}         % null space projection matrix
%\newcommand{\bc}     {\mathbf{c}}         % null space vector
%\newcommand{\dimc}   {\dimy}              % dimensionality of null space vector
%\newcommand{\bw}     {\mathbf{w}}         % image space part
%\newcommand{\dimw}   {\dimy}              %
%\newcommand{\bv}     {\mathbf{v}}         % null space part
%\newcommand{\dimv}   {\dimy}              %







% regression/classification



% generic symbols

% equations

% other





==> sections/sec3_methodology.tex <==
\section{Methodology} ~\label{sec: method}
\begin{figure*}[t!]
    \centering
    % \resizebox{0.9\textwidth}{0.35\textwidth}{%
    \includegraphics[width=0.98\textwidth]{figures/Copy of Copy of overview.png}
    % }
    \caption{Overview. }
    \label{fig:overview}
    % \vspace{-1.7em} 
\end{figure*}


In contact-rich manipulation tasks, such as assembly, robot actions are typically highly object-oriented. 
That is to say, each robot action is designed to change an object’s position, orientation, or apply an external force. 
Inspired by this observation, we use object status as a bridge between raw sensory data from demonstrations and the grounding of LLM in our project.
This formulation will help LLM...

Prior to demonstration, we construct an object-oriented skill library, where each skill corresponds to a specific change in the object’s status.
This serves as the foundation for LLM to infer current skill based on the observed status transitions during the demonstration, which are captured through the integration of multi-sensory data.
Additionally, object status also constitutes the pre- and post-condition of each skill in our skill library.
By leveraging the skill sequences learned from demonstration and associated object statuses, this formulation enables LLM to effectively plan for new task configurations, ensuring that generated plans are both executable and aligned with the intended task outcomes.

\subsection{Object-oriented Skill Library}
In our skill library, each skill is defined in an object-oriented way which describes the change of the being-manipulated object (called target object) status. \kchen{and its relation with contextual object?}
Specifically, one skill is formulated as a tuple $(O_{tar}, O_{env}, C_{pre}, C_{suc}, A, R, X, P)$. 
$O_{tar}$ represents the target object which robot directly manipulates, such as a cable or a screw. 
$O_{env}$ represents the contextual object with which the $O_{tar}$ interacts under the manipulation of robot, such as a cable clip or a socket. 
The description of other components are summarized in Table~\ref{tab: skill_form}.

\begin{table}[H]
\footnotesize
\caption{Skill Formulation}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{p{1cm}|p{5cm}|p{2cm}}
 % \hline
 % \multicolumn{10}{|c|}{Contact Change Detection Accuracy} \\
 % \hline
 % & \multicolumn{3}{|c|}{$F_c$} & \multicolumn{3}{|c|}{$df_c\symbol{92} dt$} & \multicolumn{3}{|c|}{$\rho_{c}$}\\
 % \hline
 \toprule
&Description &PDDL \\
 \hline
$O_{tar}$ &The target object which robot directly manipulates. &\texttt{parameters}\\
 \hline
$O_{env}$ &The contextual object with which the $O_{tar}$ interacts. &\texttt{parameters}\\
 \hline
$C_{pre}$ &Pre-condition. &\texttt{precondition}\\
 \hline
$C_{suc}$ &Success condition. &\texttt{effect}\\
 \hline
$A$ &The executed action connecting to low-level robot controller. &\\
 \hline
$R$ &Return. &\\
 \hline
$X$ &Skill coordinate. &\\
 \hline
$P$ &Skill parameters, including &\texttt{parameters}\\

 \bottomrule
\end{tabular}} \label{tab: skill_form}
\end{table}

Our skill library is defined originally in the formatting of code scripts.
In its construction, we create firstly a general \texttt{ObjectSkillLibrary} including skills that can be applied to all kinds of objects, such as \texttt{move} and \texttt{grasp}.
This general library is later inherited by the object-specific library which contains affordance of a specific object.
An example of \texttt{insertion} skill in \texttt{CableSkillLibrary} is shown in Listing~\ref{lst:skill_python}.
% todo: mathematical equation for functions
\begin{lstlisting}[language=Python, caption=The Insertion Skill API in Python, label={lst:skill_python}]
# The insertion skill in provided skill library.
def insert(self, direction, env_object):
    print(f"Inserting the {self.target_object} in {direction} into {env_object} and then loses contact")
    robot_controller.insert(direction, env_object)
\end{lstlisting}\kchen{should we use use different colors for prompt and answer}
By providing the object-specific skill library to the LLM, we supply explicitly $O_{tar}$ and $A$ in our skill formulation. The remaining elements, $O_{env}, C_{pre}, C_{suc}, R, X$, and $P$, are left to be completed by the LLM.

Inspired by prior works~\cite{zhou2024isr}, we first ask the LLM to translate the code scripts into a PDDL domain as a form of pre-processing to enhance the LLM's understanding of the skills and compatibility with reasoning tasks. 
In contrast to previous research, we do not actually use a PDDL planner for task planning; instead, we leverage the standard formatting and LLM's familiarity with it.
An example of the converted \texttt{insertion} skill in PDDL Domain is shown in Listing~\ref{lst:skill_pddl}.
In the translation, $C_{pre}$ and $C_{suc}$ will be completed automatically by LLM as \texttt{precondition} and \texttt{effect} in the PDDL domain.
\begin{lstlisting}[language=Python, caption=The Insertion Skill in PDDL for LLM-based Planning, label={lst:skill_pddl}]
# The insertion skill in PDDL domain traslated by LLM
(:action insert
    :parameters (?o - object ?d - direction ?e - env_object)
    :precondition (grasped ?o)
    :effect (inserted ?o ?d ?e)
  )
\end{lstlisting}

As the next step, we ask the LLM to implement the conditions generated in the PDDL domain and integrate them into the original code scripts. 
To facilitate this, we additionally provide the LLM with perception interfaces that allow it to obtain information such as robot pose, grasping status, and, importantly, proprioceptive force and torque (F/T) signals. 
While most of this information is self-explanatory, the raw F/T signals with six dimensions can be challenging for the LLM to interpret directly.
% To address this, we provide additional interfaces to obtain statistical properties of the F/T signals, such as maximum, minimum, change rate, and other relevant metrics.
To address this, without loss of generality, we assume that the task is performed in a static environment where interactions with the object occur exclusively through the robot. 
In this scenario, the most relevant F/T information will be the force or torque that opposes the robot's actions, as it provides direct feedback on the resistance encountered during manipulation.
Inspired by this observation, we reduce our F/T perception interface to include only resistance force and torque.
\begin{lstlisting}[language=Python, caption=The Insertion Skill with Post-condition Generated by LLM, label={lst:skill_post_condition}]
# The Insertion Skill API
def is_inserted(env_object, force_threshold=5.0):
    # post-condition to check if the object is inserted into the environment object
    resistance_force = perception.get_resistance_force()
    return resistance_force < force_threshold

def insert(self, direction, env_object):
    print(f"Inserting the {self.target_object} in {direction} into {env_object} and then loses contact")
    robot_controller.insert(direction, env_object, success_condition=is_inserted(env_object))
\end{lstlisting}

Listing~\ref{lst:skill_post_condition} presents an example of condition \texttt{is\_inserted} generated by LLM and its integration into the original \texttt{insert} skill.
The LLM sets the success condition for the insertion as resistance force being less than a certain threshold, which aims to detect losing contact with \texttt{env\_object} after insertion . 
Notably, since theses conditions stem from LLM's prior knowledge about the task, they might be initially inconsistent with specific task requirement or incomplete.
In the following subsection, demonstration data will be used to correct these conditions and to find appropriate threshold values. 

\subsection{Bootstrapping Reasoning of Demonstrations}
\begin{figure}[t!]
\centering
  \subfloat[]{%\begin{subfigure}[]{0.2\textwidth}
   \includegraphics[width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm },clip]{figures/method/Screenshot from compression_21_2024_05_21_26_force_tactile_post.mp4.png}
   }
   \subfloat[]{%\begin{subfigure}[]{0.2\textwidth}
   \includegraphics[width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm },clip]{figures/method/Screenshot from decompression_19_2024_05_21_12_force_tactile_post.mp4.png}
   }
   \subfloat[]{%\begin{subfigure}[]{0.2\textwidth}
   \includegraphics[ width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm },clip]{figures/method/Screenshot from linear_force_0_2024_05_21_14_force_tactile_post.mp4.png}
   }
   \subfloat[]{%\begin{subfigure}[]{0.2\textwidth}
   \includegraphics[width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{figures/method/Screenshot from rotational_force_11_2024_08_06_1_force_tactile_post.mp4.png}
   }
\caption{Tactile Signal Patterns: a) Sourcing; b) Sinking; c) Uniform Flow; d) Twisted Flow. }
\label{fig:force signal patterns}
\end{figure}

During kinesthetic demonstrations, we collect proprioceptive force measurements at the robot end effector, visual-tactile information from the robot fingers, and third-person camera images to form the demonstration data. 
Given the large volume and multiple modality of this data, it is challenging for the LLM to interpret all modalities simultaneously. 
To address this, we adopt a bootstrapping approach to prompting, where each modality is provided sequentially to assist the LLM in different stages of reasoning.
The goal of reasoning is to decompose and interpret the demonstrations into executable task plan examples.

\textbf{Multi-Modal Demonstration Segmentation} 
% Our primary insight is that tactile signal patterns have a strong correlation with subtask transitions and carry information that can be barely perceived from pure visual input in multi-step manipulation tasks, allowing for more precise identification and segmentation of these transitions. 
We obtain the initial segmentation of demonstration from transitions of $O_{tar}$ status.
As tactile information on robot fingers precepts directly the manipulation on $O_{tar}$ and carries information that can be barely perceived from the third-person camera, we rely on it for identification of status transitions.

Fig. \ref{fig:force signal patterns} illustrates four typical patterns of Vi-Tac images, each reflecting different interactions: 
a) \textit{Sourcing}: Vectors point outward, indicating a source where force radiates outward. This pattern is usually observed when grasping an object.
b) \textit{Sinking}: Vectors point inward, showing a sink where force converges inward. This pattern usually happens when releasing a grasped object.
c) \textit{Uniform Flow}: Vectors are parallel and evenly spaced, representing a consistent force in one direction. This pattern can happen when pushing or pulling the grasped object.
d) \textit{Twisted Flow}: Vectors twist gently, suggesting rotational movement around a central point. This pattern can happen when rotating or screwing the grasped object.

% We trained a dedicated classifier to accurately identify the tactile signal patterns. The classifier was fine-tuned based on the video classifier \textit{TimeSformer}\cite{gberta_2021_ICML}, with a dataset of labeled video clips collected by us.
To identify the tactile patterns above, we fine-tune a video classifier \textit{TimeSformer}~\cite{gberta_2021_ICML} with a dataset of labeled tactile videos.
Applying this classifier to demonstration will segment the complete demonstration with key timestamps when the tactile pattern changes, i.e. new events happen.
To enhance the use of tactile signals in LLM-based task planning, we further interpret these patterns from an object-centric perspective, as LLMs understand better object status semantics than abstract force patterns.
% we further correlates these tactile pattern to object status
Specifically, the four patterns—\textit{sourcing}, \textit{sinking}, \textit{uniform flow}, and \textit{twisted flow}—are mapped to object statuses of \textit{grasped}, \textit{under linear force}, \textit{under torque}, and \textit{released}, respectively.\zshen{this part might go to the beginning}

% \begin{figure*}[t!]
%     \centering
%     % \resizebox{0.9\textwidth}{0.35\textwidth}{%
%     \includegraphics[width=0.75\textwidth]{figures/method/vae.png}
%     % }
%     \caption{VAE Structure(place holder) }
%     \label{fig:vae}
%     % \vspace{-1.7em} 
% \end{figure*}

\textbf{Skill Reasoning with LLM}
After segmentation from tactile demonstration data, we provide the LLM with camera images at key timestamps (called key frames) for skill reasoning.
$O_{tar}$ and $O_{env}$ have been segmented beforehand from the task scene.
Each key frame is annotated with the corresponding $O_{tar}$ status as well as masked $O_{tar}$ and $O_{env}$. 
% feed the corresponding camera video images and object statuses into LLM to obtain a skill-based planning skeleton. % we guide the pre-trained LLM to generate step by step the executed skill sequence.
We include additionally in the prompt a simple description about the task (e.g. "two robot are mounting a cable onto several clips") and about the objects (e.g. "the blue curve in the view is the cable").
The LLM is then asked to reason which skill from the PDDL domain the robot performs at each frame.

% As the first step of reasoning, LLM maps each key frame to a skill in the initial skill domain.\zshen{better,more concise wording or abr. for skills in initial domain/in PDDL}


Although the previously genarated PDDL domain has the correct formatting, some content, such as precondition and parameters, might be inconsistent with the actual skills that we are going to run on the robots, as they are generated only from the prior knowledge of the LLM. 
Thus, as the second step, we correct and complete the PDDL domain with our demonstrations, e.g., one instance of the cable routing task. 
After correction, the LLM should be able to generate an executable plan when presented with another cable routing task in a different configuration. 

\textbf{Obtaining skill parameter and thresholds}
\subsection{Planning in New Configuration}


==> sections/sec3_skill_formulation.tex <==
\section{object-centric Skills} 
In contact-rich manipulation tasks, such as assembly, robot actions are typically highly object-centric. 
That is to say, each robot action is designed to change a certain status of an object, whether by changing its position or applying an external force.
% In the scope of our project, we focus on three key aspects of object status: positional status (including the object's position and orientation in space), force-related status (such as whether the object is subjected to external forces like pushing or pulling), and contact status (whether the object is being grasped, released, or in contact with another object or surface).
In this work, we focus on two key aspects of object status, namely, positional status (which includes the object's position and orientation) and interaction status (which describes whether the object is grasped, released, or subjected to an external force or torque).

Inspired by this fact, we construct our skill library in an object-centric manner, where each skill is defined to describe a status change of the being-manipulated object (called target object). 
In this way, the formulation of skills remains consistent whether executed by a human or a robot, enabling LLMs to generalize human demonstrations into executable task plans in new task configurations.
Additionally, we utilize the target object status as the bridge between raw sensory data from demonstrations and the grounding of LLM, which will be discussed in detail in Section~\ref{sec: reasoning}.
% Inspired by this observation, we use these object statuses as a bridge between raw sensory data from demonstrations and the grounding of LLM in our project.
% This formulation will help LLM...

\subsection{Input Skill Library}
% In our skill library, each skill is defined to describe the change of the being-manipulated object (called target object) status. 
Each skill in our skill library is formulated as a tuple $\xi = (O_{t}, O_{e}, C_{p}, C_{s}, A, R)$.
$O_{t}$ represents the target object which robot directly manipulates, such as a cable or a cap. 
$O_{e}$ represents the contextual object with which the $O_{t}$ interacts under the manipulation of robots, such as a cable clip or a bottle. 
The description and examples of all components in $\xi$ are summarized in Table~\ref{tab: skill_form}.

\begin{table}[ht]
\footnotesize
\caption{Skill Formulation}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{p{0.15cm}|p{3.8cm}|p{2.2cm}|p{1.6cm}}
 \toprule
 % \multicolumn{4}{c}{Skill Formulation} \\
 % \hline
&Description &Example &PDDL   \\
 \hline
$O_{t}$ &\textbf{Target object} that the robot directly manipulates. 
& cable &\ftnotett{parameters} \\
 \hline
$O_{e}$ &\textbf{Contextual object} with which the $O_{t}$ interacts. & clip &\ftnotett{parameters} \\
\hline
$A$ &Executed \textbf{Action} by low-level robot controller.
& insertion & \ftnotett{action} \\
 \hline
$C_{p}$ &\textbf{Pre-condition} to be met for the skill to start execution. 
& cable positioned near a clip  &\ftnotett{precondition} \\
 \hline
$C_{s}$ &\textbf{Success condition} that defines when the skill is finished. 
& cable inserted into a clip &\ftnotett{effect} \\
 \hline
$R$ & \textbf{Return} of a skill execution. & success (when $C_{s}$ is satisfied) or error & N/A\\
 \hline
% $X$ &Skill coordinate. &\\
%  \hline
$P$ &\textbf{Skill parameters}, such as force thresholds or positions. 
&position of the clip & \ftnotett{parameters}\\

 \bottomrule
\end{tabular}} \label{tab: skill_form}

\end{table}

Our skill library $L=\{\xi_i\}$, serving as input to the LLM analyzer, is defined in the form of executable code scripts.
Initially, we include object-agnostic skills, such as \smalltt{move}, in a general {\smalltt{ObjectSkillLibrary}}. 
These skills can be applied to various objects and serve as the foundation for object-specific libraries, which contain affordances of specific objects. 
For example, the \smalltt{CableSkillLibrary} includes a ``cable-centric" \smalltt{insertion} skill (see Fig.~\ref{fig:prompt_overview}(a)), which handles inserting a cable into other objects, such as clips.
The definition of each skill provides explicitly $O_{t}$ and calls the low-level \smalltt{robot\_controller} interface to perform an action $A$.
The \smalltt{robot\_controller} controls the robot to move or apply force/torque via an adaptive impedance controller~\cite{johannsmeier2019framework}.
In the following procedures, we will guide the LLM to complete the remaining components in skill $\xi$ step by step.

% Our skill library is defined originally in the formatting of code scripts.
% In its construction, we create firstly a general {\smalltt{ObjectSkillLibrary}} including skills that can be applied to all kinds of objects, such as \smalltt{move} and \smalltt{grasp}.
% This general library is later inherited by the object-specific library which contains affordance of a specific object.
% An example of \smalltt{insertion} skill in \smalltt{CableSkillLibrary} is shown in Listing~\ref{lst:skill_python}.
% By providing the object-specific skill library to the LLM, we supply explicitly $O_{t}$ and $A$ in our skill formulation. The remaining elements, $O_{e}, C_{pre}, C_{suc}, R$, and $P$, are left to be completed by the LLM.
% % todo: mathematical equation for functions
% \begin{lstlisting}[language=Python, caption=The Insertion Skill API in Python, label={lst:skill_python}]
% # The insertion skill in provided skill library.
% # This is a low-level policy
% def insert(self, direction, env_object):
%     print(f"Inserting the {self.target_object} in {direction} into {env_object} and then loses contact")
%     robot_controller.insert(direction, env_object)
% \end{lstlisting}\kchen{should we use use different colors for prompt and answer}

\subsection{Preprocessing Translation}
While the original formatting of code scripts allows skills to be executed by robots, it lacks the logic to support effective reasoning, especially conditions for skill transitions.
Inspired by prior works~\cite{silver2024generalized, zhou2024isr}, we ask the LLM analyzer to translate the input skill library into a PDDL domain as a preprocessing step.
As a standard language to describe planning problems, PDDL provides a structured syntax to represent rules like actions, objects, and conditions in its domain knowledge, which closely aligns with the composition of our input skill library.
A comparison between our skill library and the corresponding PDDL domain components is summarized in Table~\ref{tab: skill_form}.
Through translation, we aim to leverage PDDL's standard format to enhance LLMs' understanding of skills and the ability to plan for long-horizon tasks. 
As is shown in Fig.~\ref{fig:prompt_overview}(a), translation into PDDL encourages the LLM analyzer to automatically complete the transition conditions $C_{p}$ (\smalltt{precondition} in PDDL) and $C_{s}$ (\smalltt{effect} in PDDL).

% In contrast to previous research, we do not actually use a PDDL planner for task planning; instead, we leverage its standard formatting to enhance the LLM's understanding of the skills and compatibility with reasoning tasks.
% An example of the converted \smalltt{insertion} skill in PDDL Domain is shown in Listing~\ref{lst:skill_pddl}.
% In the translation, $C_{p}$ and $C_{s}$ will be completed automatically by LLM as \smalltt{precondition} and \smalltt{effect} in the PDDL domain.
% \begin{lstlisting}[language=Python, caption=The Insertion Skill in PDDL for LLM-based Planning, label={lst:skill_pddl}]
% # The insertion skill in PDDL domain traslated by LLM
% (:action insert
%     :parameters (?o - object ?d - direction ?e - env_object)
%     :precondition (grasped ?o)
%     :effect (inserted ?o ?d ?e)
%   )
% \end{lstlisting}



==> sections/sec4_reasoning.tex <==
\section{Bootstrapped Reasoning of Demonstration}\label{sec: reasoning}

\begin{figure}[t!]
\centering
\begin{tikzpicture}

    % First image
    \node at (-.5,0) {\includegraphics[width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{figures/method/Screenshot from compression_21_2024_05_21_26_force_tactile_post.mp4.png}};
    \node at (-.5,-1.0) {\footnotesize(a) grasped};

    % Second image
    \node at (1.6,0) {\includegraphics[width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{figures/method/Screenshot from decompression_19_2024_05_21_12_force_tactile_post.mp4.png}};
    \node at (1.6,-1.0) {\footnotesize(b) released};

    % Third image
    \node at (3.70,0) {\includegraphics[width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{figures/method/Screenshot from linear_force_0_2024_05_21_14_force_tactile_post.mp4.png}};
    \node at (3.7,-1.0) {\footnotesize(c) linear force};

    % Fourth image
    \node at (5.80,0) {\includegraphics[width=0.24\columnwidth, trim={1.8cm 1.8cm 1.8cm 1.8cm},clip]{figures/method/Screenshot from rotational_force_11_2024_08_06_1_force_tactile_post.mp4.png}};
    \node at (5.80,-1.0) {\footnotesize(d) torque};
\end{tikzpicture}
\vspace{-1.7em}
\caption{Tactile Signal Patterns and Corresponding Object Statuses: (a) Sourcing pattern, referring to "grasped" status; (b) Sinking, referring to "released" status; (c) Uniform Flow, referring to "under a linear force" status; (d) Twisted Flow, referring to "under torque" status.}
\label{fig:force signal patterns}
\vspace{-1.5em}
\end{figure}


% During demonstrations, we collect proprioceptive force measurements at the robot end effector, visual-tactile information from the robot fingers, and third-person camera images to form the demonstration data. 
% Following the object-centered skill library, we use these object statuses as a bridge between raw sensory data from demonstrations and the grounding of LLM in our project.
Given the large volume and multi-modal nature of our demonstration data, it can be challenging for LLMs to interpret all modalities simultaneously. 
To address this problem, we adopt a bootstrapped approach for in-context learning of demonstration, where each modality is introduced sequentially to assist the LLM in different stages of reasoning.
Tactile information is utilized to segment events from visual perception and identify object statuses, which then enables LLMs to comprehend the entire demonstration and infer the corresponding skill sequence $S_d = (\xi_1, \xi_2, ...)$. 
Afterwards, F/T signals are leveraged to ground and refine the transition conditions between skills ensuring that the learned skill sequence are executable and can generalize to new task scenarios by re-planning.

\subsection{Segmentation with Object Status} 
% Our primary insight is that tactile signal patterns have a strong correlation with subtask transitions and carry information that can be barely perceived from pure visual input in multi-step manipulation tasks, allowing for more precise identification and segmentation of these transitions. 
To facilitate skill reasoning from demonstration data, we first segment the entire demonstration into events where object status changes.
We rely on tactile status for this segmentation, as tactile information on robot fingers directly precepts the manipulation on target object $O_{t}$, thus capturing details that are often missed by third-person cameras.

Fig. \ref{fig:force signal patterns} illustrates four typical patterns of Vi-Tac images, each reflecting different interaction status of the target object: 
a) \textit{Sourcing}: Vectors point outward, indicating a source where force radiates outward. This pattern is usually observed when an object is ``grasped".
b) \textit{Sinking}: Vectors point inward, showing a sink where force converges inward, usually when a grasped object is ``released".
c) \textit{Uniform Flow}: Vectors are parallel and evenly spaced, representing a consistent force in one direction. This pattern happens when an object is ``under a linear force", such as being pushed or pulled.
d) \textit{Twisted Flow}: Vectors twist gently, suggesting rotational movement around a central point. This pattern happens when an object is ``under torque", such as being rotated or screwed.

To identify the above tactile patterns in demonstrations, we fine-tune the video classifier \textit{TimeSformer}~\cite{gberta_2021_ICML} with a dataset of labeled tactile videos.
% We segment the complete demonstration with the classifier into events when the tactile pattern changes, i.e., new interaction happens. 
Applying this classifier to the complete demonstration then segments it into events when new interaction happens.
Object status alongside the timestamps of these events (referred to as key timestamps) are extracted for subsequent reasoning.
% To enhance the use of tactile signals in LLM-based task planning, we further interpret these patterns from an object-centric perspective, as LLMs understand better object status semantics than abstract force patterns.
% Specifically, the four patterns—\textit{sourcing}, \textit{sinking}, \textit{uniform flow}, and \textit{twisted flow}—are mapped to object statuses of \textit{grasped}, \textit{under linear force}, \textit{under torque}, and \textit{released}, respectively.\zshen{this part might go to the beginning}

% \begin{figure*}[t!]
%     \centering
%     % \resizebox{0.9\textwidth}{0.35\textwidth}{%
%     \includegraphics[width=0.75\textwidth]{figures/method/vae.png}
%     % }
%     \caption{VAE Structure(place holder) }
%     \label{fig:vae}
%     % \vspace{-1.7em} 
% \end{figure*}

\subsection{Skill Reasoning with LLM}
% Beforehand, the objects involved in the task are segmented from the scene, and their properties—such as position, orientation, and particularly the opening direction for the clips—are stored in a scene database. 
After segmentation, we provide the LLM analyzer with camera images taken at key timestamps (referred to as key frames) for skill reasoning. 
As is shown in Fig.~\ref{fig:prompt_overview} (a), each key frame is annotated with objects as well as the the corresponding status of $O_{t}$.
Additionally, we include in the prompt a simple description of the task (e.g., ``two robots are mounting a cable onto several clips") and of the objects (e.g., ``the blue curve in the view is the cable"). 
% feed the corresponding camera video images and object statuses into LLM to obtain a skill-based planning skeleton. % we guide the pre-trained LLM to generate step by step the executed skill sequence.
The LLM is then asked to reason which skill from the PDDL domain the demonstrator has performed at each key timestamp.

% \begin{lstlisting}[caption= An Excerpt of Skill Sequence Reasoned by the LLM from Demonstration, label={lst: reasoning}]
% Frame 1: (move_object clip8); Because one of the robots is moving with the cable towards the position of clip 8

% Frame 2: (grasp cable); Because the tactile status indicates the cable is grasped

% Frame 3: (stretch cable); Because the tactile status indicates the cable is under linear force, suggesting a stretching action

% Frame 4: (insert cable clip8); Because the tactile status indicates the cable is under torque, suggesting an insertion action into clip 8
% \end{lstlisting}
Fig.~\ref{fig:prompt_overview}(b) presents an example of the skill sequence reasoned by the LLM. 
We observe that the LLM adaptively utilizes camera images (for \smalltt{move\_object}) and object status (for \smalltt{grasp}, \smalltt{stretch}, and \smalltt{insert}) to infer the corresponding skills. 
In addition, the LLM also fills in the contextual object $O_e$ (\smalltt{env\_object}) for each skill in its reasoning.

% Afterwards, we also provide an interface to read from the scene database, where properties (such as position and orientation) of all contextual objects $O_{e}$ are stored. 
% Integrating these object data with the previous answer will result in 

% As is shown in Listing~\ref{lst: object_property}, this allows the LLM to expand the skill sequence with specific parameters $P$, such as \smalltt{pose} in \smalltt{move\_object} and \smalltt{direction} in \smalltt{insert}.
% \begin{lstlisting}[language=Python, caption= An Excerpt of Skill Sequence Expanded with Scene Objects, label={lst: object_property}]
% cable_skill_library.move_object(get_object_property('clip8', 'position'))
% cable_skill_library.grasp()
% cable_skill_library.stretch()
% cable_skill_library.insert(get_object_property('clip8', 'insertion_direction'), 'clip8')
% cable_skill_library.open_hand()
% \end{lstlisting}


% As the first step of reasoning, LLM maps each key frame to a skill in the initial skill domain.\zshen{better,more concise wording or abr. for skills in initial domain/in PDDL}

% Although the previously genarated PDDL domain has the correct formatting, some content, such as precondition and parameters, might be inconsistent with the actual skills that we are going to run on the robots, as they are generated only from the prior knowledge of the LLM. 
% Thus, as the second step, we correct and complete the PDDL domain with our demonstrations, e.g., one instance of the cable routing task. 
% After correction, the LLM should be able to generate an executable plan when presented with another cable routing task in a different configuration. 

\subsection{Skill Conditions with LLM}
The final step in converting the skill sequence into an executable task plan is to reason about success conditions for each skill. 
We leverage the \smalltt{precondition} and \smalltt{effect} in the previously translated PDDL domain.
The LLM is requested to implement these conditions and integrate them back into the skill library. 
Additionally, we provide the LLM with interfaces to access perception information about robot pose, grasping status, and F/T signals. 
Since most of the other information is either binary or straightforward when used to form conditions (e.g. whether an object is grasped or a position is reached), we focus especially on F/T conditions which are highly variable and crucial for contact-rich manipulations.

The raw six-dimensional F/T signals are complex for the LLM to interpret directly.
To address this without sacrificing generality, we assume that the task is performed in a static environment where interactions with the object occur exclusively through the robot. 
In this context, the most relevant F/T information pertains to the force or torque opposing the robot's actions, as they provide direct feedback on the resistance encountered during manipulation.
Based on this observation, we reduce our F/T perception interface to include only resistance force $f_r$ and torque $\tau_r$.

For each skill, we first ask the LLM to generate an initial success condition function, in which it determines which signal the condition should be based on (e.g. \smalltt{resistance\_torque} is used to form the \smalltt{is\_tightened} condition). 
A plot of the selected signal is then provided and the LLM is prompted to update the success condition function accordingly.
An example of the resulting condition \smalltt{is\_inserted} for the task of mounting cable to clips is shown in Fig.~\ref{fig:prompt_overview} (c). 
The LLM defines the success condition for insertion as the resistance force falling below a certain threshold, indicating that the cable has been securely inserted. 
We present later in Section~\ref{subsec: reason_eval} that numerical thresholds are particularly refined with the provided F/T signals.
% With the aid of the plot, the LLM also selects an appropriate value for the threshold.
% \begin{lstlisting}[language=Python, caption=The Insertion Skill with Post-condition Generated by LLM, label={lst: skill_post_condition}]
% # Based on the plot, the resistance torque increases 
% # significantly during the tightening process, reaching 
% # values above 1.0 N. To ensure the cap is tightened, we 
% # can set a threshold slightly below the peak torque
% # observed in the demonstration.
% ...

% def is_tightened(threshold=1.0):
%     # post-condition to check if the object is tightened
%     resistance_torque = perception.get_resistance_torque()
%     return resistance_torque > threshold
% ...

% def tighten(self):
%     print(f"Tighten the {self.target_object}")
%     robot_controller.screw(success_condition=lambda: is_tightened())
% \end{lstlisting}
% Listing~\ref{lst:skill_post_condition} presents an example of condition \smalltt{is\_inserted} generated by LLM and its integration into the original \smalltt{insert} skill.
% The LLM sets the success condition for the insertion as resistance force being less than a certain threshold, which aims to detect losing contact with \smalltt{env\_object} after insertion. 
% Notably, since theses conditions stem from LLM's prior knowledge about the task, they might be initially inconsistent with specific task requirement or incomplete.
% In the following subsection, demonstration data will be used to correct these conditions and to find appropriate threshold values. 

\subsection{Planning on New Scenarios}
From the above bootstrapping reasoning, the LLM analyzer has extracted the skill sequences  corresponding to human demonstrations, and has extended the original skill library with appropriate success conditions.
These outputs are then combined as an demonstration task plan, which will be used as an example for task planning on a new task.
As shown in Fig~\ref{fig: overview}, in the planning request to an LLM planner, we include the demonstration task plan as well as an image and description of the new task scene.
% Given the large impact the demonstration task plan will bring to the planner, the generated new plan might highly duplicates the one in demonstration.
To make the plan more dynamic and flexible, we also use the LLM planner to monitor the execution process.
After execution of each skill, we feed its return $R$ back to the LLM planner, which then decides whether the plan should be continued or adjusted.


